Inductive Certificate Synthesis for Control Design

The focus of this thesis is developing a framework for designing correct-by-construction controllers using control certificates. We use nonlinear dynamical systems to model the physical environment (plants). The goal is to synthesize controllers for these plants while guaranteeing formal correctness w.r.t. given specifications. We consider different fundamental specifications including stability, safety, and reach-while-stay. Stability specification states that the execution traces of the system remain close to an equilibrium state and approach it asymptotically. Safety specification requires the execution traces to stay in a safe region. Finally, for reach-while-stay specification, safety is needed until a target set is reached. The design task consists of two phases. In the first phase, the control design problem is reduced to the question of finding a control certificate. More precisely, the goal of the first phase is to define a class of control certificates with a specific structure. This definition should guarantee the following: "Having a control certificate, one can systematically design a controller and prove its correctness at the same time." The goal in the second phase is to find such a control certificate. We define a potential control certificate space (hypothesis space) using parameterized functions. Next, we provide an inductive search framework to find proper parameters, which yield a control certificate. Finally, we evaluate our framework. We show that discovering control certificates is practically feasible and demonstrate the effectiveness of the automatically designed controllers through simulations and real physical systems experiments.

==> synt/barrier.tex <==
\subsection{Barrier Certificates}
The safety problem can be reduced to the problem of
finding a (relaxed~\cite{prajna2004safety}) control barrier certificate $B$ which respect 
the following constraints~\cite{WIELAND2007462}:
\begin{equation}\label{eq:barrier-cert-def} 
\begin{array}{rl}
(\forall \vx \in I) \ & B(\vx) < 0 \\
(\forall \vx \not\in int(S)) \ & B(\vx) > 0 \\
(\forall \vx \in S \setminus int(I)) \ (\exists \vu \in U)\ & \nabla B \cdot f(\vx, \vu) < 0 \,. \\ 
\end{array}
\end{equation}
To find such a barrier certificate, one needs to define $B$ as a linear
combination of basis functions and use the framework to find a correct $B$.
The verifier would check the following conditions that negate each of the
conditions in Eq.~\eqref{eq:barrier-cert-def}.
First we check if there is a $\vx \in I$ such that $B(\vx) \geq 0$.
\[
 (\exists \vx)\ \ \bigwedge_{j=1}^l p_{I,j}(\vx) \leq 0 \ \land\ B(\vx) \geq 0\,.
\]

Next, we check if there exists a $\vx \not \in int(S)$ such that $B(\vx) \leq 0$. Clearly, if $\vx \not\in int(S)$, we have $p_{S,i}(\vx) \geq 0$ for at least one $i \in \{1,\ldots,k\}$. This yields $k$ conditions of the form:
\[
  (\exists \vx) \ p_{S,i}(\vx) \geq 0 \land B(\vx) \leq 0,\ i \in \{ 1, \ldots, k\}\,.
\]
Finally, we ask if $\exists \vx \in S \setminus int(I)$ that violates the decrease condition. Doing so, we obtain $l$ conditions. For each $i \in \{ 1, \ldots, l \}$, we solve
\begin{align*}
(\exists \vx) & \ \underset{\vx \not\in int(I)}{\underbrace{p_{I,i}(\vx) \geq 0}} \land\ \underset{\vx \in S}{\underbrace{\bigwedge_{j=1}^k p_{S,j}(\vx) \leq 0}} \\
	     &\ \land (\forall \vu \in U) \ \nabla B \cdot f(\vx, \vu) \geq 0 \,,
\end{align*}

Overall, we have $1 + k + l$ different checks. If any of these checks result
in $\vx$, it serves as a counterexample to the conditions for a barrier function
~\eqref{eq:barrier-cert-def}.

As before, we choose basis functions $g_1, \ldots, g_r$ for the barrier
set $B_\vc: \sum_{j=1}^r c_j g_j(\vx)$.
% Notice that for example, for the first condition in 
% Eq.~\eqref{eq:barrier-cert-def} a counterexample $\vx$ has to satisfy $\vx \in I$.
Given observations set $O_j: \{ (\vx_1, \vu_1), \ldots, (\vx_{j-1}, \vu_{j-1})\}$, the corresponding
 candidate set $C_j$ of observation compatible barrier functions
is defined as the following:
\[
C_j: \left\{ \vc |\hspace{-0.1cm}
\begin{array}{l}
\bigwedge\limits_{(\vx_i, \vu_i) \in O_j}
\left(\begin{array}{rl} 
\vx_i \in I \rightarrow & B_\vc(\vx_i) < 0 \ \land \\
\vx_i \not\in int(S) \rightarrow & B_\vc(\vx_i) > 0 \ \land \\
\vx_i \in S\setminus int(I)& \\ \rightarrow \nabla B_\vc & . f(\vx_i, \vu_i)<0 \end{array}\right)\end{array}\right\}.
\]
The LHS of the implication for each observation $(\vx_i, \vu_i)$ is evaluated
 and the RHS constraint is added only when the LHS holds. Nevertheless, $\overline{C_j}$ remains a polytope similar to Lemma.~\ref{lemma:cj-convex}. 

 



==> synt/constraint_solving.tex <==
\section{Constraint Solvers}
The constraints we are interested in solving are defined over a real domain. Given a set of vector variables $\vx$ and set of \emph{hard} constraint
\[
h_i(\vx), (i \in \{1,\ldots,M\} \,,
\]
we wish to either find a feasible solution $\vx^*$, or prove that no $\vx^*$ exists.

\paragraph{Linear Programming}
When the constraints are linear in $\vx$, i.e. $h_i(\vx): \va_i \cdot \vx \geq b_i$, then, the problem is a linear programming (LP) problem. Efficient methods exist for solving such problems~\todo{cite}. In addition, we use the following theorem which lies at the heart of convex optimization.
\begin{theorem}[Farkas Lemma for LP~\todo{cite}]\label{thm:farkas}
Exactly one of the following holds:
\begin{compactitem}
	\item $(\exists \vx) \ A \vx \leq \vb$
	\item $(\exists \vlam) \ \vlam \geq \vzero \,, \vb^t\vlam < 0 \,, A^t \vlam = \vzero$.
\end{compactitem}
or alternatively:
\begin{compactitem}
	\item $(\exists \vx) \ \vx > \vzero \,, A \vx = \vb$
	\item $(\exists \vlam) \ A^t \vlam \geq \vzero \,, \vb^t\vlam \leq 0$.
\end{compactitem}
\end{theorem}
In addition to feasibility check, one could also optimize some objective function for these cases (in case a feasible solution exists).

\paragraph{Semi-definite Programming}
A more general problem is to solve for linear matrix inequality constraints. More specifically, the variables form a square and symmetric matrix $X$, and there are two type of constraints: (i) linear constraints, and (ii) one LMI constraint which requires $X$ to be positive semi-definite. In other words:
\begin{align*}
h_1(X) &: X \succeq 0 \\
h_i(X) &: \tupleof{A_i, X} \leq b_i , (i \in \{2,\ldots,M\})\,,
\end{align*}
where $\tupleof{A, B}$ is the trace of inner product of $A$ and $B$.
The constraints here yield a convex feasible set. As such, global solution is effectively computable. 

\begin{theorem}[Farkas Lemma for SDP~\todo{cite}]\label{thm:farkas-sdp}
Exactly one of the following holds:
\begin{itemize}
	\item $X \succ 0 \,, \bigwedge_i \tupleof{A_i, X} = b_i$
	\item $\vzero \neq \sum_i A_i^t \vlam \succeq 0 \,, \vb^t \vlam \leq 0$
\end{itemize}
\end{theorem}
As a corollary, one can show for a give $C \succ 0$:
\[
(\forall X \succeq 0, \neq \vzero) \ \tupleof{C, X} > 0 \ \ \ \mbox{or} \ \ \ (\forall \vx \neq \vzero) \ \tupleof{C, \vx \vx^t} > 0
\]

\paragraph{Non Convex Problems}
When the set of feasible solutions is not convex, the problem is known to be harder and there are sets of solutions to address such problems. 

In the first approach, first-order or second-order methods are used to find a locally optimal solution, by optimizing an objective function. However, a locally optimal solution may not be a feasible solution. This method is used for solving bilinear problems such as BMI~\cite{el1994synthesis}, nonlinear MPC~\todo{cite}, and deep neural networks~\todo{cite}.

In the second set of solutions, instead of a local optimal solution, we wish to find a global one. One could SMT solvers. The constraints are quantifier free if they only involve boolean operators and nonlinear (strict) inequalities. This class of constraints are Quantifier Free Nonlinear Real Arithmetic (QFNRA) formulae.

. However, these methods are known to suffer from curse of dimensionality as they may recursively decompose the search space into smaller cells. If the only source of non-convexity is boolean disjunctions and all the terms are linear, then the problem belongs to ``linear real arithmetic" theory ($\scr{LRA}$):
\[
g_i(\vx) : \bigvee_j \  \va_{ij} \cdot \vx \leq b_{ij} \,. 
\]
Otherwise, it belongs to ``nonlinear real arithmetic" theory ($\scr{NRA}$).




==> synt/disturbance.tex <==
\subsection{Disturbances}

We will now extend the original CEGIS framework to handle these
further quantifier alternations. The idea is conceptually simple: we
will extend the witnesses structure.  Rather than
witnesses which are simply points $\vx_i \in X$, we will
now allow witnesses that are of the form $(\vx_i, (Q \mapsto D) )$,
i.e, a combination of a state $\vx_i \in X$ and a map from each mode
to a disturbance vector. Since $Q$ is finite, this map is explicitly
stored as $(\vx_i, (q_1, \vd_1), \ldots, (q_m,\vd_m))$.

First, we note that the RCLF requirements yield formulae of the form
\[ (\exists\ \vc)\ (\forall\ \vx) \Psi(\vc,\vx) \,,\]
but $\Psi$ itself is a quantified formula with the following structure:
\begin{equation}\label{eq:cegis-form-dist}
\bigwedge\ \begin{cases}
	\vx \in R_1 \implies \bigvee_q (\forall\ \vd)\ p_{1,q}(\vc,\vx,\vd) < 0 \\
	\vx \in R_2 \implies \bigvee_q (\forall\ \vd)\ p_{2,q}(\vc,\vx,\vd) < 0 \\
	\vdots \\
	\vx \in R_r \implies \bigvee_q (\forall\ \vd)\ p_{r,q}(\vc,\vx,\vd) < 0\,.
\end{cases}
\end{equation}


A first solution consists of applying CEGIS for $\exists\forall$
described previously. However, doing so yields quantified constraints
for the candidate and witness generation steps. Since our objective
was to avoid these quantified constraints in the first place, we modify
the witness structure.

\paragraph{Witness Structure:} As mentioned earlier, a witness to the
violation of a given RCLF candidate $\vc \in C$ include a state
$\vx \in X$ at which the violation happens along with for each mode
$q_j$ that can be selected for the mode, a disturbance witness
$\vd_j \in D$ that will violate the formula.
With disturbances, each witness then has the following structure:
\begin{equation}\label{eq:witness-structure}
 \vy_i:\ \left( \vx_i, (q_1, \vd^{(i)}_{1}), \ldots, (q_m, \vd^{(i)}_{m}) \right) \,.
\end{equation}
With this witness structure, the overall CEGIS procedure now extends naturally.

\paragraph{Candidate Generation:} Let $\mathcal{Y}_n: \{ \vy_1,\ldots,\vy_n \}$ be the set of witnesses
at the $n^{th}$ iteration, starting from $\mathcal{Y}_0: \emptyset$. The candidate
is generated by solving the formula: 
\begin{equation}\label{eq:cegis-candidate-gen-inst}
 \psi_n[\vc]:\ (\vc \in C)\ \land\ \bigwedge_{i=1}^n \mathsf{inst}(\Psi,\vy_i) \,, 
\end{equation}
wherein $ \mathsf{inst}(\Psi,\vy_i)$ substitutes the witness from Eq.~\eqref{eq:witness-structure}
for the variables $\vx$, $q$, $\vd$ in Eq.~\eqref{eq:cegis-form-dist}.
\begin{equation}\label{eq:cegis-instantiation-dist}
\mathsf{inst}(\Psi,\vy_i):\ \begin{cases}
 \bigvee_{k=1}^m p_{1,q_k}(\vc,\vx_i,\vd^{(i)}_k) < 0 \\
 \bigvee_{k=1}^m p_{2,q_k}(\vc,\vx_i,\vd^{(i)}_k) < 0 \\
	\vdots \\
\bigvee_{k=1}^m p_{r,q_k}(\vc,\vx_i,\vd^{(i)}_k) < 0 \,. \\
\end{cases}
\end{equation}
We now use an SMT solver to find if the unquantified formula $\psi_n$ from
Eq.~\eqref{eq:cegis-candidate-gen-inst}.

\paragraph{Witness Generation:} Once a candidate $\vc = \vc_n$ is generated by
solving $\psi_n$, we now evaluate if it is a true RCLF. This involves, substituting
$\vc_n$ for $\vc$ in formula $\Psi$ in Eq.~\eqref{eq:cegis-form-dist} and checking
if $\lnot \Psi$ is satisfiable.  Since $\Psi$ itself is the conjunction of $r> 0$
conditions, its negation is a disjunction and we can check each disjunct separately
for satisfiability.  Each disjunct has the following form:
\[ \vx \in R_j\ \land\ \bigwedge_{k=1}^m\ (\exists\ \vd \in D)\
p_{j,q_k}(\vc_n, \vx, \vd) \geq 0 \,.\]
We can remove the existential quantifier over $\vd$ equivalently thr-ough 
$m= |Q|$ fresh set of variables $\vd_1, \ldots, \vd_m$. The new disjunct
is written:
\begin{equation}\label{eq:witness-generation-rclf-form}
 \vx \in R_j\ \land\ \bigwedge_{k=1}^m p_{j,q_k}(\vc_n,\vx,\vd_k) \geq 0 \,. 
\end{equation}
If satisfiable, we obtain a witness $(\vx_{n+1}, (q_1, \vd^{(n+1)}_1),\ldots, (q_m,$ $\vd^{(n+1)}_m) )$.
Otherwise, we conclude that $\vc_n$ represents a valid RCLF.

==> synt/inductive.tex <==
\section{Inductive Synthesis}





==> synt/multiple.tex <==
\subsection{Multiple Barriers}
We now explain the CEGIS
framework that searches for a suitable control certificate $V$. To
synthesize a control certificate, we start with a parametric form
$V_\vc(\vx) = V(\vc,\vx): \sum_{i=1}^N c_i g_i(\vx)$ with some 
(nonlinear) basis functions
$g_1(\vx),$ \ldots $, g_N(\vx)$ chosen by the user, and unknown
coefficients $\vc:\ (c_1,$ \ldots $, c_N)$, s.t. $\vc \in C$ for a compact set $C \subseteq \reals^N$. The certificate $V$ is a linear function over $\vc$.

The constraints from Eq.~\eqref{eq:rws-basic-exp} become as follows:
\begin{equation}\label{eq:template-rws-basic-exp}
\begin{array}{l}
(\exists \vc \in C) \ (\forall \vx \in X) \ \vx \in S \setminus G \implies \bigvee_q 
\left(
\dot{V_q}<-\epsilon\land
 \bigwedge_{j \in J_q} \left( \dot{p_{S,j,q}}(\vx) + \lambda p_{S,j}(\vx)<-\epsilon \right)
\right) \,.
	
\end{array}
\end{equation}

The constraints in Eq.~\eqref{eq:template-rws-basic-exp} has a complex
quantifier alternation structure involving the $\exists \vc$
quantifier nested outside the $\forall \vx$ quantifier.  First, we note that
$J_q$ is computed separately and here we assume it is given. Next, we modify an
algorithm commonly used for program synthesis problems to the problem
of synthesizing the coefficients $\vc \in C$~\cite{solar2008program}.


The counterexample guided inductive synthesis (CEGIS) approach has its
roots in program synthesis, wherein it was proposed as a general
approach to solve $\exists \forall$ constraints that arise in such
problems~\cite{solar2008program}.  The key idea behind the CEGIS
approach is to find solutions to such constraints while using a
satisfiability (feasibility) solver for quantifier-free formulas that
check whether a given set of constraints without quantifiers have a
feasible solution.

Solvers like Z3 allow us to solve many different classes of
constraints with extensive support for linear arithmetic
constraints~\cite{DeMoura-Bjorner-08-Z3}.  On the other hand, general
purpose nonlinear delta-satisfiability solvers like dReal, support the
solving of quantifier-free nonlinear constraints involving
polynomials, trigonometric, and rational
functions~\cite{DBLP:conf/cade/GaoKC13}. However, the presence of quantifiers
drastically increases the complexity of solving these
constraints. Here, we briefly explain the idea of CEGIS procedure for
$\exists\forall$ constraints of the form
\[ (\exists\ \vc \in C)\ (\forall\ \vx \in X)\ \Psi(\vc,\vx) . \]
Here, $\vc$ represents the unknown coefficients of a control
certificate and $\vx$ represents the state variables of the system.
Our goal is to find one witness for $\vc$ that makes the overall
quantified formula true. The overall approach constructs, maintains,
and updates two sets iteratively:
\begin{enumerate}

\item $X_i \subseteq X $ is a finite set of \emph{witnesses}. This is explicitly represented as $X_i = \{ \vx_1, \ldots, \vx_i \}$.
\item $C_i \subseteq C$ is a (possibly infinite) subset of  available \emph{candidates}. This is implicitly represented by a constraint $\psi_i(\vc)$, s.t.
$C_i:\ \{ \vc\ \in C\ |\ \psi_i(\vc) \}$.
\end{enumerate}

In the beginning, $X_0 = \{ \}$
and $\psi_0:\ \true$ representing the set $C_0:\ C$.

At each iteration, we perform the following steps:

\noindent (a) \emph{Choose} a
candidate solution $\vc_{i+1} \in C_i$. This is achieved by checking
the feasibility of the formula $\psi_i$. Throughout this paper, we
will maintain $\psi_i$ as a \emph{linear arithmetic} formula that
involves boolean combinations of linear inequality
constraints. Solving these problems is akin to solving linear
optimization problems involving disjunctive constraints. Although the
complexity is NP-hard, solvers like Z3 integrate fast LP solvers with
Boolean satisfiability solvers to present efficient solutions~\cite{DeMoura-Bjorner-08-Z3}.

\noindent (b) \emph{Test} the current candidate. This is achieved by
testing the satisfiability of $ \lnot \Psi(\vc, \vx)$ for fixed
$\vc = \vc_{i+1}$. In doing so, we obtain a set of nonlinear constraints
over $\vx$. We wish to now check if it is feasible.

If $\lnot \Psi(\vc_{i+1},\vx)$ has no feasible solutions, then
$\Psi(\vc_{i+1},\vx)$ is true (valid) for all $\vx$. Therefore, we can
stop with $\vc = \vc_{i+1}$ as the required solution for $\vc$.

Otherwise, if $\lnot \Psi(\vc, \vx)$ is feasible for some $\vx= \vx_{i+1}$,
we add it back as a witness: $X_{i+1}:\ X_i \cup \{ \vx_{i+1}\}$. The
formula $\psi_{i+1}$ is given by
\[ \psi_{i+1}:\ \psi_i\ \land\ \Psi(\vc, \vx_{i+1}) \,.\]
Note that $\psi_{i+1}\ \implies\ \psi_i$, and $\vc_{i+1}$ is no longer
a feasible point for $\psi_{i+1}$.  The set $C_{i+1}$ described by
$\psi_{i+1}$ is:
\[ C_{i+1}:\ \{ \vc \in C\ |\ \Psi(\vc,\vx_i)\ \mbox{holds for each}\ \vx_i \in X_{i+1} \} \,.\]


The CEGIS procedure either (i) runs forever, or (ii) terminates after
$i$ iterations with a solution $\vc: \vc_{i}$, or (iii) terminates
with a set of witness points $X_i$ proving that no solution exists. 

We now provide further details of the CEGIS procedure adapted to find
a certificate that satisfies Eq.~\eqref{eq:template-rws-basic-exp}. In
the CEGIS procedure, the formula $\Psi(\vc, \vx)$ will have the following form:
\begin{equation}
\label{eq:phi}
\begin{cases}
	\vx \in R_1 \implies \varphi_1(\vc, \vx) \\
	\vx \in R_2 \implies \varphi_2(\vc, \vx) \\
	... \\
	\vx \in R_{N_j} \implies \varphi_{N_j}(\vc, \vx) \,,
\end{cases}
\end{equation}
and each $\varphi_j$ for $j = 1,\ldots, N_j$ has the form 
\begin{equation} \label{eq:phi-k-finite}
\bigvee_k \bigwedge_l \ p_{j,k,l}(\vc, \vx) > 0 \,,
\end{equation}
where $p_{j,k,l}(\vc, \vx)$ is a function linear in $\vc$ and possibly nonlinear in $\vx$, depending on the dynamics and template used for the control certificate. 
%
%\begin{remark}
%	Our previous framework in~\cite{Ravanbakhsh-Others/2015/Counter}
%        deals only with conditions where $\varphi_k$ has the form
%        $\bigvee_i p_{k,j}(\vc, \vx) > 0$.  The extension to the form
%        in Eq.~\eqref{eq:phi-k-finite} is described here for completeness.
%\end{remark}

The CEGIS procedure involves two calls to solvers: (a) Testing
satisfiability of $\psi_i(\vc)$ and (b) Testing the satisfiability of
$ \lnot \Psi(\vc_{i+1}, \vx)$. We shall discuss each of these problems
in the following paragraphs.

\paragraph{Finding Candidate Solutions:}
Given a finite set of witnesses $X_i$, a solution exists for
$\psi_{i+1}$ iff there exists $\vc \in C$ s.t. 
%for all $\vx \in X_i$ and $1 \leq k \leq N_k$ 
\begin{equation*} \bigwedge_{\vx \in
X_i} \ \bigwedge_{j=1}^{N_j} \left( \vx \in R_j \implies \bigvee_k \bigwedge_l
p_{j,k,l}(\vc, \vx) > 0 \right)\,, \end{equation*} and since $p_{j,k,l}$ is a linear function in $\vc$, such $\vc$ can be found by solving a formula in Linear Arithmetic Theory ($\scr{LA}$).


\paragraph{Finding Witnesses:} Finding a witness for a given candidate solution $\vc_i$ involves checking the satisfiability $\lnot \Psi$. Whereas $\Psi$ is a
conjunction of $N_j$ clauses, $\lnot \Psi$ is a disjunction of
clauses.  The $j^{th}$ clause in $\lnot \Psi$ ($1 \leq j \leq N_j$) has the form 
\begin{equation} \label{eq:ce-piece} \vx \in
R_j \land \bigwedge_k \bigvee_l p_{j,k,l}(\vc_i, \vx) \leq 0 \, . \end{equation}

We will test each clause separately for satisfiability.
Assuming that $p_{j,k,l}$ is a general nonlinear function over $\vx$, SMT solvers like dReal~\cite{DBLP:conf/cade/GaoKC13} can be used to solve this over a compact set $R_j$.  Numerical SMT
solvers like dReal can either conclude that the given formula is
unsatisfiable or provide a solution to a ``nearby'' formula that is
$\delta$ close. The parameter $\delta$ is adjusted by the user. As a result, dReal can correctly conclude that the current
candidate yields a valid certificate.  On the other hand, its witness
may not be a witness for the original problem. In this case, using the
spurious witness may cause the CEGIS procedure to potentially continue
(needlessly) even when a solution $\vc_i$ has been
found. Nevertheless, the overall procedure produces a correct result
whenever it terminates with an answer.

==> synt/rws.tex <==
\subsection{Lyapunov-Barrier Certificates}

In this problem, the goal is to reach a target set $T$ from an initial
set $I$, while staying in a safe set $S$, wherein
  $I \subseteq S$. The set $S$ is assumed to be compact.  By
combining the local Lyapunov function and a barrier certificate, one
can define a smooth, Lyapunov-like
function $V$, that satisfies the following conditions
(see~\cite{ravanbakhsh2016robust}):

\begin{equation}\label{eq:lyapunov-like-def} 
  \begin{array}{lrl}
C1:&(\forall \vx \in I) & V(\vx) < 0 \\
C2:&(\forall \vx \not\in int(S)) & V(\vx) > 0 \\
C3:&(\forall \vx \in S \setminus int(T)) (\exists \vu \in U)& \nabla V \cdot f(\vx,\vu)\hspace{-0.05cm}<\hspace{-0.05cm}0. \\ 
\end{array}
\end{equation}

 We briefly sketch the argument as to why such a Lyapunov-like
  function satisfies the reach-while-stay, referring the
  reader to our earlier work on control certificates for a detailed
  proof~\cite{ravanbakhsh2016robust}.  Suppose we have found
  a function $V$ satisfying~\eqref{eq:lyapunov-like-def}.  $V$ is
  strictly negative over the initial set $I$ and strictly positive
  outside the safe set $S$.  Furthermore, as long as the flow remains
  inside the set $S$ without reaching the interior of the target $T$,
  there exists a control input at each state to strictly decrease the
  value of $V$.  Combining these observations, we conclude either (a)
  the flow remains forever inside set $S \setminus int(T)$ or (b) must visit the
  interior of set $T$ (before possibly leaving $S$). However, option (a) is ruled
  out because $S \setminus int(T)$ is a compact set and $V$ is a continuous
  function. Therefore, if the flow were to remain within $S \setminus int(T)$ forever
  then $V(\vx(t)) \rightarrow -\infty$ as $t \rightarrow \infty$,
  which directly contradicts the fact that $V$ must be lower bounded
  on a compact set $S \setminus int(T)$. We therefore, conclude that the flow must stay
  inside $S$ and eventually visit the interior of the target $T$.  

The learning framework extends easily to search for a function $V$
that satisfies the constraints in Eq.~\eqref{eq:lyapunov-like-def}.

\input{synt/disturbance}


\subsection{Control Funnels}
The idea of funnels has been developed to use the Lyapunov argument
for time-varying regions of invariance for a finite horizon~\cite{mason1985mechanics}.
Then, following Majumdar et al., a library of
control funnels can provide building blocks for motion
planning~\cite{majumdar2013control}. Likewise, control funnels are used to
reduce reach-avoid problem to timed automata~\cite{bouyer2017timed}.


  In this section, we consider Lyapunov-like functions for establishing
  control funnels.  Let $I$ be a set of initial states for the plant ($\vx(0) \in I$),
  and $T$ be the target set that the system should reach at time $\T > 0$ ($\vx(\T) \in int(T)$).
  Let $S$ be the safe set, such that $I, T \subseteq S$
  and $\vx(t) \in S$ for time $t \in [0,\T]$. The goal is to find a controller
  that guarantees that whenever $\vx(0) \in I$, we have $\vx(t) \in S$ for
  all $t \in [0, \T]$ and $\vx(\T) \in int(T)$. To solve this, we search instead
  for a control Lyapunov-like function $V(\vx,t)$ that is a function of
  the state and time, with the following properties:

\begin{equation}\label{eq:c-funnel-def} 
\begin{array}{lrl}
C1:& (\forall \vx \in I) & V(\vx, 0) < 0 \\
C2:& (\forall \vx \not\in int(T)) & V(\vx, \T)\ > \ 0 \\
C3:& \left(\forall \begin{array}{l}t \in [0, \T] \\ 
		\vx \not\in int(S) \end{array}\right) & V(\vx, t) > 0 \\
C4:&\left(\begin{array}{l}\forall t \in [0, \T]\\ 
		\forall \vx \in S\end{array}\right) (\exists \vu \in U)& \dot{V}(t, \vx, \vu) < 0 \,,\\ 
\end{array}
\end{equation}
where $\dot{V}(t, \vx, \vu) = \frac{\partial V}{\partial t} + \nabla V \cdot f(\vx, \vu)$.
First of all, when initialized to $\vx(0) \in I$, we have $V(\vx,0) < 0$ by condition
  C1. Next, the controller's action through condition $C4$ guarantees that $\frac{dV}{dt} < 0$ over the
  trajectory for $t \in [0, \T]$, as long as $\vx \in S$. Through $C3$, we can guarantee that $\vx(t) \in S$ for
  $t \in [0,\T]$. Finally, it follows that $V(\vx(\T),\T) < 0$. Through $C2$, we conclude that
  $\vx \in int(T)$. 
As depicted in Fig.~\ref{fig:funnel}, the set $V^{=0}$ forms a barrier, and set $V^{<0}$ 
forms the required funnel, while $t \leq \T$.

Using the Lyapunov-like conditions~\eqref{eq:c-funnel-def}, the
problem of finding such control funnels (respecting
Eq.~\eqref{eq:c-funnel-def}) belongs to the class of problem which
could be solved with our method.

\input{synt/multiple}

